Compositional Obverter Communication Learning From Raw Visual Input

One of the distinguishing aspects of human language is its compositionality, which allows us to describe complex environments with limited vocabulary. Previously, it has been shown that neural network agents can learn to communicate in a highly structured, possibly compositional language based on disentangled input (e.g. hand- engineered features). Humans, however, do not learn to communicate based on well-summarized features. In this work, we train neural agents to simultaneously develop visual perception from raw image pixels, and learn to communicate with a sequence of discrete symbols. The agents play an image description game where the image contains factors such as colors and shapes. We train the agents using the obverter technique where an agent introspects to generate messages that maximize its own understanding. Through qualitative analysis, visualization and a zero-shot test, we show that the agents can develop, out of raw image pixels, a language with compositional properties, given a proper pressure from the environment.

==> background.tex <==
\subsection{Emergence of grammar}
In \citet{batali1998computational}, the author successfully trained neural agents to develop a compositional language using disentangled meaning vectors as the input.
Using 10 subject vectors and 10 predicate vectors, all represented as explicit binary vectors, total 100 meaning vectors could be composed (see Table~\ref{tab:meaning_vectors} in Appendix~\ref{supp:batali_tables}).
The author used twenty neural agents for the experiment.
Each agent was implemented with the vanilla recurrent neural networks (RNN), where the hidden vector $\hb$'s size was 10, same as the size of the meaning vector $\mb$ in order to treat $\hb$ as the agent's \textit{understanding} of $\mb$.

In each training round a single learner (\textit{i.e.} listener) and ten teachers (\textit{i.e.} speaker) were randomly chosen.
Each teacher, given all 100 $\mb$'s in random order, generates a message $\sbb$\footnote{A message is a sequence of alphabets chosen from \textit{a, b, c} or \textit{d}. The maximum length was set to 20.} for each $\mb$ and sends it to the learner. 
%The learner's $\hb$, after consuming the message $\sbb$, will have changed to some value.
The learner is trained to minimize the mean squared error (MSE) between $\hb$ (after consuming the $\sbb$) and $\mb$.
After the learner has learned from all ten teachers, the next round begins, repeating the process until the error goes below some threshold.
When the training was complete, the author was able to find compositional patterns in the messages used by the agents (see Table~\ref{tab:batali_analysis} in Appendix~\ref{supp:batali_tables}).

Note that we have not mentioned how the teacher generates a message $\sbb$ given a meaning vector $\mb$. In fact, next subsection is dedicated to describing how messages are generated using the simple yet elegant technique named \textit{obveter}.

\subsection{Obverter technique}
\citet{batali1998computational} used the \textit{obverter} technique to train the neural agents, which has its root in the theory of mind. Theory of mind~\citep{premack1978does} observes that a human has direct access only to one's own mind and not to the others'. Therefore we typically assume that the mind of others is analogous to ours, and such assumption is reflected in the functional use of language~\citep{bruner1981intention}. For example, if we want to convey a piece of information to the listener\footnote{We assume the listener cannot speak but only listen. Therefore the listener's mind is completely hidden.}, it is best to speak in a way that maximizes the listener's understanding. However, since we cannot directly observe the listener's state of mind, we cannot exactly solve this optimization problem. Therefore we posit that the listener's mind operates in a similar manner as ours, and speak in a way that maximizes \textit{our understanding}, thus approximately solving the optimization problem. This is exactly what the obverter technique tries to achieve.

In each round, the teacher (\textit{i.e.} speaker), given a meaning vector $\mb$, generates a message using its own RNN. 
%to send to the learner (\textit{i.e.} listener), using its own RNN, of which the hidden vector $\hb$ can be viewed as the teacher's mind.
After initializing its hidden vector $\hb$ to zeros, the teacher greedily selects a symbol at each timestep that modifies $\hb$ as close to $\mb$ as possible. The selected symbol is appended to the message, and the hidden vector induced by that symbol is used in the next timestep. This continues until either the message length reaches the predefined maximum, or the difference between $\hb$ and $\mb$ goes below some threshold (see the detailed algorithm in Appendix~\ref{supp:batali_algorithm}). Therefore the teacher, through introspection, generates a message that maximizes its own understanding (\textit{i.e.} $\hb$ becomes similar to $\mb$), hoping that the same message will also make sense to the learner. We remind the reader that only the learner's RNN parameters are updated, and the teacher uses its fixed RNN. Therefore an agent uses only one RNN for both speaking and listening, guaranteeing self-consistency (see Appendix~\ref{supp:reinforce_comparison} for a detailed comparison between the obverter technique and the RL-based approach).
%and they learn to communicate by learning to be a good listener

Another feature of the obverter technique is that it observes the \textit{principle of least effort}~\citep{zipf2016human}. Because the teacher stops generating symbols as soon as $\hb$ and $\mb$ become similar enough, it does not waste any more effort trying to \textit{perfect} the message. The same principle was implemented in one way or another in previous works, such as choosing the shortest among the generated strings~\citep{kirby2002emergence} or imposing a small cost for generating a message~\citep{mordatch2017emergence}. 
%On a side note, \citet{batali1998computational}'s obverter technique was motivated by a simpler message generation technique named \textit{Saussurean}, which was used by \citet{hurford1989biological} for sending a single-character message. We can see that both techniques are strongly rooted in the theory of mind and the human development of language, although we cannot say for certain whether the authors had such theory in mind.

==> batali_comp.tex <==
\begin{table}[h]
% \small
\centering
\begin{subfigure}{\textwidth}
\centering
\captionsetup{width=.7\linewidth}
\begin{footnotesize}
\begin{tabular}{l|llllllllll}
\hline
\textit{-} & \textit{one} & \textit{they} & \textit{you} & \textit{yall} & \textit{yup} & \textit{me} & \textit{we} & \textit{mip} & \textit{yumi} & \textit{all} \\
\hline
\textit{tired} & cda & cdab & cdc & cdcb & cdba & cd & cdd & cddb & cdcd & cdb\\
\textit{scared} & caa & caab & cac & cacb & caba & ca & cad & cadb & cacd & cab\\
\textit{sick} & daa & daab & dac & dacb & daba & da & dad & dadb & dacd & dab\\
\textit{happy} & baa & baab & bca & bcab & baac & ba & badc & bab & bac & babc\\
\textit{sad} & aba & abab & ac & acb & abac & a & abdc & abb & abc & abbc\\
\textit{excited} & cba & cbab & cca & cacb & cbca & c & ccdc & cb & ccb & cbc\\
\textit{angry} & bb & bbb & bc & bcb & bbc & b & bddc & bdb & bdc & bdbc\\
\textit{silly} & aa & aaab & aca & acab & adba & add & addc & adad & adc & adbc\\
\textit{thirsty} & dbaa & dbab & dca & dcba & dbca & dda & ddac & dbad & dcad & dbacd\\
\textit{hungry} & dbb & dbbd & dc & dcb & dbc & dd & ddc & dbd & dcd & dbcd\\
\hline
\end{tabular}
\end{footnotesize}
%\caption{Messages most often used by the two agents when speaking about a given object. Brackets indicate variations often seen in the messages.}
%\label{tab:two_factors_messages}
\end{subfigure}

\vspace*{5mm}
\begin{subfigure}{\textwidth}
\centering
\captionsetup{width=.7\linewidth}
\begin{footnotesize}
\begin{tabular}{l|llllllllll}
\hline
\textit{-} & \textit{one} & \textit{they} & \textit{you} & \textit{yall} & \textit{yup} & \textit{me} & \textit{we} & \textit{mip} & \textit{yumi} & \textit{all} \\
\hline
\textit{tired} & {- -}a & {- -}ab & {- -}c & {- -}cb & {- -}ba & {- -} & {- -}d & {- -}db & {- -}cd & {- -}b\\
%\textit{tired} & \texttt{--}a & \texttt{--}ab & \texttt{--}c & \texttt{--}cb & \texttt{--}ba & \texttt{--} & \texttt{--}d & \texttt{--}db & \texttt{--}cd & \texttt{--}b\\
\textit{scared} & {- -}a & {- -}ab & {- -}c & {- -}cb & {- -}ba & {- -} & {- -}d & {- -}db & {- -}cd & {- -}b\\
%\textit{scared} & \texttt{--}a & \texttt{--}ab & \texttt{--}c & \texttt{--}cb & \texttt{--}ba & \texttt{--} & \texttt{--}d & \texttt{--}db & \texttt{--}cd & \texttt{--}b\\
\textit{sick} & {- -}a & {- -}ab & {- -}c & {- -}cb & {- -}ba & {- -} & {- -}d & {- -}db & {- -}cd & {- -}b\\
%\textit{sick} & \texttt{--}a & \texttt{--}ab & \texttt{--}c & \texttt{--}cb & \texttt{--}ba & \texttt{--} & \texttt{--}d & \texttt{--}db & \texttt{--}cd & \texttt{--}b\\
\textit{happy} & {- -}a & {- -}ab & {-}c{-} & {-}c{-}b & {- -}ac & {- -} & {- -}dc & {- -}b & {- -}c & {- -}bc\\
%\textit{happy} & \texttt{--}a & \texttt{--}ab & \texttt{-}c\textit{-} & \texttt{-}c\texttt{-}b & \texttt{--}ac & \texttt{--} & \texttt{--}dc & \texttt{--}b & \texttt{--}c & \texttt{--}bc\\
\textit{sad} & {-}ba & {-}bab & {-}c & {-}cb & {-}bac & {-} & {-}bdc & {-}bb & {-}bc & {-}bbc\\
%\textit{sad} & \texttt{-}ba & \texttt{-}bab & \texttt{-}c & \texttt{-}cb & \texttt{-}bac & \texttt{-} & \texttt{-}bdc & \texttt{-}bb & \texttt{-}bc & \texttt{-}bbc\\
\textit{excited} & {-}ba & {-}bab & {-}ca & {-}acb & {-}bca & {-} & {-}cdc & {-}b & {-}cb & {-}bc\\
%\textit{excited} & \texttt{-}ba & \texttt{-}bab & \texttt{-}ca & \texttt{-}acb & \texttt{-}bca & \texttt{-} & \texttt{-}cdc & \texttt{-}b & \texttt{-}cb & \texttt{-}bc\\
\textit{angry} & {-}b & {-}bb & {-}c & {-}cb & {-}bc & {-} & {-}ddc & {-}db & {-}dc & {-}dbc\\
%\textit{angry} & \texttt{-}b & \texttt{-}bb & \texttt{-}c & \texttt{-}cb & \texttt{-}bc & \texttt{-} & \texttt{-}ddc & \texttt{-}db & \texttt{-}dc & \texttt{-}dbc\\
\textit{silly} & (aa) & (aaab) & (aca) & (acab) & {- -}ba & {- -}d & {- -}dc & {- -}ad & {- -}c & {- -}bc\\
%\textit{silly} & (aa) & (aaab) & (aca) & (acab) & \texttt{--}ba & \texttt{--}d & \texttt{--}dc & \texttt{--}ad & \texttt{--}c & \texttt{--}bc\\
\textit{thirsty} & {-}b{-}a & {-}b{-}b & {-}c{-} & {-}cb{-} & {-}bc{-} & {-}d{-} & {-}d{-}c & {-}b{-}d & {-}c{-}d & {-}b{-}cd\\
%\textit{thirsty} & \texttt{-}b\texttt{-}a & \texttt{-}b\texttt{-}b & \texttt{-}c\texttt{-} & \texttt{-}cb\texttt{-} & \texttt{-}bc\texttt{-} & \texttt{-}d\texttt{-} & \texttt{-}d\texttt{-}c & \texttt{-}b\texttt{-}d & \texttt{-}c\texttt{-}d & \texttt{-}b\texttt{-}cd\\
\textit{hungry} & {-}bb & {-}bbd & {-}c & {-}cb & {-}bc & {-}d & {-}dc & {-}bd & {-}cd & {-}bcd\\
%\textit{hungry} & \texttt{-}bb & \texttt{-}bbd & \texttt{-}c & \texttt{-}cb & \texttt{-}bc & \texttt{-}d & \texttt{-}dc & \texttt{-}bd & \texttt{-}cd & \texttt{-}bcd\\
\hline
\end{tabular}
\end{footnotesize}
%\caption{Potential analysis of the messages in terms of prefixes and suffixes.}
%\label{tab:two_factors_analysis}
\end{subfigure}
%\caption{Messages most often used by the two agents when speaking about a given object. Brackets indicate variations often seen in the messages.}
\caption{(Top) Messages used by a majority of the population for each of the given meanings. (Bottom) A potential analysis of the system in terms of a root plus modifications. Sequences in parentheses cannot be made to fit into this analysis.}
\label{tab:batali_analysis}
\end{table}

==> comp_diagonal_alt_bak.tex <==
\begin{table}[h]
% \small
\centering
\begin{subfigure}{\textwidth}
\centering
\captionsetup{width=.7\linewidth}
\begin{footnotesize}
\begin{tabular}{l|l|l|l|l|l}
\hline
\textbf{-} & \textbf{Box} & \textbf{Sphere} & \textbf{Cylinder} & \textbf{Capsule} & \textbf{Ellipsoid} \\
\hline
\textbf{Blue} & \cellcolor{light_gray}eeeeeee\{e,ee\} & eeeeee & eeeeee\{e,ed\} & eeee\{e,ed\} & eee\{e,a\}\\
\textbf{Red} & ee\{e,a\} & \cellcolor{light_gray}e,ea & e\{e,a\} & {b,ba} & {a,c}\\
\textbf{White} & {bbbbb} & {bb} & \cellcolor{light_gray}{bbb\{b,d\}} & {bb\{b,d\}} & {bbb\{d,c\}}\\
\textbf{Gray} & {eeee} & {e,ea} & {ee\{e,a\}} & \cellcolor{light_gray}{e,a} & {b,d}\\
\textbf{Yellow} & {bb\{c,d\}} & {e\{e,ec\}} & {b\{c,d\}} & {a,c} & \cellcolor{light_gray}{a,e}\\
\textbf{Green} & {eeeeee\{e,a\}} & {eeee\{e,a\}} & {eeeee\{e,a\}} & {eee\{e,a\}} & {ee\{e,a\}}\\
\textbf{Cyan} & {eeeeeeeeea,a$\times$20}  & {eeeeee\{e,a\}} & {eeeeeee\{e,ea\}} & {eeeee\{e,a\}} & {eeeea}\\
\textbf{Magenta} & {bbb\{b,d\}} & {c,d} & {bb\{b,d\}} & {bb} & {b\{c,a\}}\\
\hline
\end{tabular}
\end{footnotesize}
\end{subfigure}

\vspace*{3mm}
\begin{subfigure}{\textwidth}
\centering
\captionsetup{width=.7\linewidth}
\begin{footnotesize}
\begin{tabular}{l|l|l|l|l|l}
\hline
\textbf{-} & \textbf{Box} & \textbf{Sphere} & \textbf{Cylinder} & \textbf{Capsule} & \textbf{Ellipsoid} \\
\hline
\textbf{Blue} & \cellcolor{light_gray}\textit{eeeeee} {e\{e,ee\}} & \textit{eeee} {ee} & \textit{eeeee} {e\{e,ed\}} & \textit{eee} {e\{e,ed\}} & \textit{ee} {e\{e,a\}}\\
\textbf{Red} & \textit{eeeeee} {\={e}\={e}\={e}\={e}\{e,a\}} & \cellcolor{light_gray}\textit{eeeeee} {\={e}\={e}\={e}\={e}\{e,ea\}} & \textit{eeeee} {\={e}\={e}\={e}\={e}\{e,a\}} & \textit{eee} {\={e}\={e}\={e}\={e}\{b,ba\}} & \textit{ee} {\={e}\={e}\={e}\={e}\{a,c\}} \\
\textbf{White} & \textit{bbbb} {b} & \textit{b} {b} & \cellcolor{light_gray}\textit{bbb} {\{b,d\}} & \textit{bb} {\{b,d\}} & \textit{bbb} {\{d,c\}}\\
\textbf{Gray} & \textit{eeeeee} {\={e}\={e}\={e}e} & \textit{eeee} {\={e}\={e}\={e}\{\_,a\}} & \textit{eeeee} {\={e}\={e}\={e}\{e,a\}} & \cellcolor{light_gray}\textit{eee} {\={e}\={e}\={e}\{e,a\}} & \textit{ee} {\={e}\={e}\={e}\{b,d\}} \\
\textbf{Yellow} & \textit{bbbb} {\={b}\={b}\{c,d\}} & \textit{b} {\={b}\={b}e\{e,ec\}} & \textit{bbb} {\={b}\={b}\{c,d\}} & \textit{bb} {\={b}\={b}\{a,c\}} & \cellcolor{light_gray}\textit{bbb} {\={b}\={b}\{a,e\}}\\
\textbf{Green} & \textit{eeeeee} {\{e,a\}} & \textit{eeee} {\{e,a\}} & \textit{eeeee} {\{e,a\}} & \textit{eee} {\{e,a\}} & \textit{ee} {\{e,a\}}\\
\textbf{Cyan} & \textit{eeeeee} {eeea} & \textit{eeee} {ee\{e,a\}} & \textit{eeeee} {ee\{e,ea\}} & \textit{eee} {ee\{e,a\}} & \textit{ee} {eea}\\
\textbf{Magenta} & \textit{bbbb} {\={b}\{b,d\}} & \textit{b} {\={b}\{c,d\}} & \textit{bbb} {\={b}\{b,d\}} & \textit{bb} {\={b}b} & \textit{bbb} {\={b}\={b}\{c,a\}}\\
\hline
\end{tabular}
\end{footnotesize}
\end{subfigure}
\caption{(Top) Messages most often used by the two agents when speaking about a given object. Shaded cells indicate the objects not seen during the training. Brackets indicate the variation often seen at the last character. 
(Bottom) Potential analysis of the messages. \textit{Italic} symbols are used to specify shapes and roman symbols are used to specify colors. \={b} indicates a single deletion of \textit{b}. \={e} indicates a single deletion of \textit{e}.}
\label{tab:two_factors_diagonal_analysis}
\end{table}

==> exp_two_factors.tex <==
\begin{figure}[t]
\centering
%\begin{subfigure}{.7\textwidth}
%\centering
%\includegraphics[width=\textwidth]{figs/progress_0}
%\end{subfigure}
%
%\begin{subfigure}{.7\textwidth}
%\centering
%\includegraphics[width=\textwidth]{figs/progress_1}
%\end{subfigure}
\includegraphics[width=.7\textwidth]{figs/progress}
\caption{Progress during the training. (Top) We plot the training accuracy, training loss, average message length (divided by maximum length, 20) in the round and average message distinctness in the round. (Bottome) We plot the perplexities (divided by 20) and the Jaccard similarity of the messages spoken by both agents in the round.}
\label{fig:training_progress}
\end{figure}

\input{table_f2.tex}

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{figs/visual_tsne}
\caption{t-SNE plots of the ConvNet's output features.}
\label{fig:visual_tsne}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{figs/blue_box}
\caption{Ten communication examples when the speaker is given a blue box.  Five examples on the left show when the listener is given blue objects. Five examples on the right show when the listener is given objects of different colors.}
\label{fig:blue_box}
\end{figure}

\input{table_f2_diagonal.tex}

==> old_exp_two_factors.tex <==
\input{table_two_factors_comp.tex}

\subsection{Two Factors: Color and Shape of Objects}
\label{ssec:two_factors}
Here we describe the results from the experiment with images containing two factors, namely eight colors and five shapes.
We have conducted the following four variants of zero-shot evaluation with trained agents.
\begin{itemize}[leftmargin=5.5mm]
\item \textbf{Diagonal}: We can make a matrix with eight rows (\textit{i.e.} colors) and five columns (\textit{i.e.} shapes).
When training the agents to communicate, we leave out the diagonal elements: blue box, red sphere, white cylinder, gray capsule, yellow ellipsoid. At the testing phase, we see if the agents can successfully communicate given the held-out images.
\item \textbf{No Blue}: When training the agents, we leave out the blue color, so that the agents are allowed to observe only four colors and eight shapes.
At the testing phase, we see if the agents can successfully communicate given the new color, blue.
\item \textbf{No Box}: When training the agents, we leave out the box shape, so that the agents are allowed to observe only seven shapes and five colors.
At the testing phase, we see if the agents can successfully communicate given the new shape, box.
\item \textbf{No Blue \& No Box}: When training the agents, we leave out the both the blue color and the box shape, so that the agents are allowed to observe only seven shapes and four colors.
At the testing phase, we see if the agents can successfully communicate given the new shape and the new color, namely box and blue.
\end{itemize}

\subsubsection{Zero-shot: Diagonal}
\textbf{Sanity check}: Before evaluating the zero-shot performance, we first test the trained agents whether they have learned the general concept of color and shape, rather than memorizing the images in the training set.
We therefore test the agents with newly generated off-diagonal objects, which they have not seen during training.
Note that in this sanity check, the test images do not include the held-out diagonal elements.

The best performing agents demonstrated the final training accuracy of 0.965\footnote{This was calculated with the last minibatch during the training process}.
We tested them with 1,000 new images where the test accuracy was 0.963. 
Therefore we can safely say that the agents have learned the general knowledge of shape and color.
%The color-specific, shape-specific accuracy is described in Table \ref{tab:specific_accuracy}.
%Figures show several examples.
%\input{specific_accuracy_tab.tex}

\begin{figure}[t]
\centering
\begin{subfigure}{.5\textwidth}
	\centering\captionsetup{width=.9\linewidth}%
	\includegraphics[width=.9\textwidth]{./figs/red_box_1}
	\caption{Red box is described as 0,0,0,0}
    \label{fig:red_box_1}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
	\centering\captionsetup{width=.9\linewidth}%
	\includegraphics[width=.9\textwidth]{./figs/red_box_2}
	\caption{Red box is described as 1,(6),0,0,6,-}
    \label{fig:red_box_2}
\end{subfigure}
\caption{Communication examples when the speaker is given a red box.
The first column shows the images given to the speaker.
The second column shows the images given to the listener.
The last column shows the plot where the x-axis is the number of characters consumed by the listener, y-axis the score produced by the listener.
From the top to the bottom, each row shows when the agents are given the same object, objects of the same shape, objects of the same color, different objects.}
\label{fig:red_box}
\end{figure}

\edward{Some analysis.}

For all future experiments, we skip the sanity check and discuss the results of zero-shot tests.

\textbf{Zero-shot test}: We now investigate the agents' performance when held-out diagonal elements are introduced.
Note that we use the same newly generated images from the previous sanity check, but this time we include the held-out diagonal elements.
This test set of images will be used for all following evaluation.
The communication accuracies for four cases are described in Table \ref{tab:zeroshot_diagonal}.
The marginal differences of accuracy in four columns show that the agents adapt surprisingly well to the objects that they have never seen during training.

\begin{table}
% \small
\caption{Communication accuracy for \textit{diagonal zero-shot} test. The first column describes the mean accuracy when both the teacher and the learner are given one of the held-out objects. The second column is for when only the teacher is given one of the held-out objects, and so forth. The value inside the parenthesis indicates the number of samples among the entire 1,000 test image pairs.}
\centering
\begin{footnotesize}
\begin{tabular}{c|c|c|c|c}
\textbf{-} & \textbf{Teacher \& Learner} & \textbf{Teacher only} & \textbf{Learner only} & \textbf{None} \\
\toprule
\textbf{Accuracy} & 0.978261 (56) & 0.968254 (71) & 0.949367 (66) & 0.963054 (807) \\
\bottomrule
\end{tabular}
\end{footnotesize}
\label{tab:zeroshot_diagonal}
\end{table}

\begin{figure}[t]
\centering
\includegraphics[width=.45\textwidth]{./figs/white_cylinder}
\caption{Four communication examples of white cylinder, one of the diagonal elements.
The first row shows a successful communication, even though the agents have never seen it during training. 
The second and third row shows the difference a single character can make.
By adding a single character \textit{8}, the speaker makes it clear that he is referring to a white cylinder.
The last row shows a mistake made by the speaker. 
7,7,1,8 is agents usually use for referring to a green cylinder.
Therefore the listener naturally produces a high score.}
\label{fig:white_cylinder_diagonal}
\end{figure}


\edward{Some figures and analysis}

\subsubsection{Zero-shot: No blue}
We investigate the agents' performance when the held-out blue objects are introduced.
The communication accuracies for four cases are described in Table \ref{tab:zeroshot_noblue}.

\begin{table}
% \small
\caption{Communication accuracy for \textit{no blue zero-shot} test. The description for the columns are the same as Table \ref{tab:zeroshot_diagonal}.}
\centering
\begin{footnotesize}
\begin{tabular}{c|c|c|c|c}
\textbf{-} & \textbf{Teacher \& Learner} & \textbf{Teacher only} & \textbf{Learner only} & \textbf{None} \\
\toprule
\textbf{Accuracy} & 1.0 (72) & 0.911111 (45) & 0.975610 (41) & 0.979810 (842) \\
\bottomrule
\end{tabular}
\end{footnotesize}
\label{tab:zeroshot_noblue}
\end{table}

\edward{Some figures and analysis}

\subsubsection{Zero-shot: No box}
We investigate the agents' performance when the held-out box objects are introduced.
The communication accuracies for four cases are described in Table \ref{tab:zeroshot_nobox}.

\begin{table}
% \small
\caption{Communication accuracy for \textit{no box zero-shot} test. The description for the columns are the same as Table \ref{tab:zeroshot_diagonal}.}
\centering
\begin{footnotesize}
\begin{tabular}{c|c|c|c|c}
\textbf{-} & \textbf{Teacher \& Learner} & \textbf{Teacher only} & \textbf{Learner only} & \textbf{None} \\
\toprule
\textbf{Accuracy} & 0.921739 (115) & 0.750000 (80) & 0.750000 (88) & 0.953975 (717) \\
\bottomrule
\end{tabular}
\end{footnotesize}
\label{tab:zeroshot_nobox}
\end{table}

\begin{figure}[t]
\centering
\includegraphics[width=.45\textwidth]{./figs/red_box_no_box}
\caption{Four communication examples of a red box.
The agents have never seen a box during training.
The agents are having difficulty sending consistent messages for the same object.}
\label{fig:red_box_no_box}
\end{figure}


\edward{The agents are having a hard time because they are often confused with box and cylinders. Considering the robust performance in the previous section, this implies that the agents handle colors more effectively than shapes.}

\subsubsection{Zero-shot: No blue \& no box}
We investigate the agents' performance when blue objects and box objects are introduced.
The communication accuracies for four cases are described in Table \ref{tab:zeroshot_noblue_nobox}.

\begin{table}
% \small
\caption{Communication accuracy for \textit{no blue \& no box zero-shot} test. The description for the columns are the same as Table \ref{tab:zeroshot_diagonal}.}
\centering
\begin{footnotesize}
\begin{tabular}{c|c|c|c|c}
\textbf{-} & \textbf{Teacher \& Learner} & \textbf{Teacher only} & \textbf{Learner only} & \textbf{None} \\
\toprule
\textbf{Accuracy} & 0.949749 (199) & 0.842105 (95) & 0.807692 (104) & 0.983389 (602) \\
\bottomrule
\end{tabular}
\end{footnotesize}
\label{tab:zeroshot_noblue_nobox}
\end{table}

\edward{Some figures and analysis}




==> old_experiment.tex <==
\subsection{Experiment setup}
\begin{itemize}
\item two-factor experiment
\begin{itemize}
\item floor color variation
\item vocab size variation
\item tying the convnet params(?)
\end{itemize}
\item three-factor experiment: tentative experiment with the best performing setup
\end{itemize}

\subsection{Implementation details}
Talk about hyperparameters, hardware, running time, etc.

\subsection{Evaluation setup}
Due to recent development of this project, I need to re-write the experiments section.
\begin{itemize}
\item Compositionality analysis (Increasing allowed characters)
\item 2D visualization of ConvNet features (Maybe talk about the disentangled nature of the features)
\item Zero-shot performance analysis
\item Training for 3 factors (color, shape, number)
\end{itemize}

\input{exp_two_factors.tex}

\begin{figure}[t]
\centering
\caption{t-SNE plots of the ConvNet's output features.}
\label{fig:visual_tsne}
\includegraphics[width=\textwidth]{figs/visual_tsne}
\end{figure}

\subsection{Evaluation Strategy}
It is not a trivial task to quantitatively evaluate the compositionality of the communication. Unlike classification or prediction tasks where one would typically use evaluation metrics such as accuracy or AUC, there is no straightforward way to report that the messages were $x\%$ compositional. 
In \citet{batali1998computational}, the author conducted an analysis on the messages sent between the agents to see if the messages were following any pattern. He also conducted a zero-shot task where the agents were not exposed to some meaning vectors during the training phase, and tested with the held-out meaning vectors during the test phase.

In our work, in order to evaluate the linguistic aspect of the agents, we conduct the same pattern analysis and zero-shot tests for both two-factor experiments and three-factor experiments. In addition, since the agents in our setup learns visual cognition as well as the linguistic capability, we study if the ConvNet component of the agent has learned to recognize objects in the image and effectively differentiate between different objects. 

If the agents truly are using compositional language, then they must be able to describe things they have not seen before.
For example, if the agents can describe blue box and red sphere in a compositional manner, they should be able to describe red box, even though they have never seen it before.
In section \ref{ssec:two_factors}, we discuss results from experiments with two factors: shape and color of objects.
In section \ref{ssec:three_factors}, we discuss results from experiments with three factors: shape, color and the number of objects.
In all evaluation, two agents change the speaker/listener role ten times, each time using 100 images pairs as the minibatch.
We use the same minibatch ratio described in section \ref{ssec:training_strategy}.
Based on the successful/failed binary prediction using 0.5 as the threshold, we calculate the mean communication accuracy.

\subsection{Three Factors: Color, Shape and Number of Objects}
\label{ssec:three_factors}
After seeing the success in handling two factors, we push the boundary and include one more factor: the number of objects.
In addition to eight colors and five shapes, there can be either one object or two objects in the image.
We conducted two versions of experiments as follows:
\begin{itemize}[leftmargin=5.5mm]
\item \textbf{Easy Three Factors}: Only the same type can be coupled. Therefore there are 80 varieties in total (40 different objects $\times$ one/two objects).
\item \textbf{Hard Three Factors}: Any two types can be coupled. Therefore there are 1600 varieties in total (40 different objects $\times$ 40 different objects). \edward{Todo}
\end{itemize}
For both versions, we conduct the \textit{diagonal zero-shot} evaluation. In addition to the diagonal elements described in the previous section, we add two blue spheres for \textit{easy three factors}. For \textit{hard three factors}, we add two blue spheres, one red box and one red ellipsoid, one white box and one black box, one yellow box and one green sphere.

\subsubsection{Easy three factors, diagonal zero-shot}
We investigate the agents' performance when the diagonal elements including two blue spheres are introduced.
The communication accuracies for four cases are described in Table \ref{tab:easy_three_factors}.

\begin{table}
% \small
\caption{Communication accuracy for \textit{easy three factors, diagonal zero-shot} test. The description for the columns are the same as Table \ref{tab:zeroshot_diagonal}.}
\centering
\begin{footnotesize}
\begin{tabular}{c|c|c|c|c}
\textbf{-} & \textbf{Teacher \& Learner} & \textbf{Teacher only} & \textbf{Learner only} & \textbf{None} \\
\toprule
\textbf{Accuracy} & 0.875000 (24) & 0.942308 (52) & 0.983051 (59) & 0.922543 (865) \\
\bottomrule
\end{tabular}
\end{footnotesize}
\label{tab:easy_three_factors}
\end{table}

\edward{Some figures and analysis}

==> old_table_f2_analysis_16760.tex <==
\begin{table}[h]
% \small
\centering
\begin{subfigure}{\textwidth}
\centering
\captionsetup{width=.7\linewidth}
\begin{footnotesize}
\begin{tabular}{l|l|l|l|l|l}
\hline
\textbf{-} & \textbf{Box} & \textbf{Sphere} & \textbf{Cylinder} & \textbf{Capsule} & \textbf{Ellipsoid} \\
\hline
\textbf{Blue} & {bbbbbbb\{b,d\}} & {bb\{b,d\}} & {bbbbbb\{b,d\}} & {bbbbb\{c,d\}} & {bbbb\{\_,c,d\}}\\
%\textbf{Blue} & \texttt{bbbbbbb\{b,d\}} & \texttt{bb\{b,d\}} & \texttt{bbbbbb\{b,d\}} & \texttt{bbbbb\{c,d\}} & \texttt{bbbb\{\_,c,d\}}\\
\textbf{Red} & {aaaa\{c,e\}} & {aa\{c,e\}} & {aaa\{c,e\}} & {a\{c,e\}} & {c,e}\\
%\textbf{Red} & \texttt{aaaa\{c,e\}} & \texttt{aa\{c,e\}} & \texttt{aaa\{c,e\}} & \texttt{a\{c,e\}} & \texttt{c,e}\\
\textbf{White} & {bbbbbb} & {b,d} & {bbbb\{b,d\}} & {bbb\{b,d\}} & {bb\{\_,c,d\}}\\
%\textbf{White} & \texttt{bbbbbb} & \texttt{b,d} & \texttt{bbbb\{b,d\}} & \texttt{bbb\{b,d\}} & \texttt{bb\{\_,c,d\}}\\
\textbf{Gray} & {aaa} & {a} & {aa} & {c} & {b,bd}\\
%\textbf{Gray} & \texttt{aaa} & \texttt{a} & \texttt{aa} & \texttt{c} & \texttt{b,bd}\\
\textbf{Yellow} & {aaaaaa} & {aaaa} & {aaaaa} & {aaa} & {a\{a,e\}}\\
%\textbf{Yellow} & \texttt{aaaaaa} & \texttt{aaaa} & \texttt{aaaaa} & \texttt{aaa} & \texttt{a\{a,e\}}\\
\textbf{Green} & {aaaa\{a,ad\}} & {aa\{a,ad\}} & {aaa\{a,ad\}} & {a\{a,ad\}} & {a}\\
%\textbf{Green} & \texttt{aaaa\{a,ad\}} & \texttt{aa\{a,ad\}} & \texttt{aaa\{a,ad\}} & \texttt{a\{a,ad\}} & \texttt{a}\\
\textbf{Cyan} & {a$\times$20} & {bbb\{b,d\}} & {bbbbbbb\{b,d\}} & {bbbbbbd} & {bbbbb\{b,d\}}\\
%\textbf{Cyan} & \texttt{a$\times$20} & \texttt{bbb\{b,d\}} & \texttt{bbbbbbb\{b,d\}} & \texttt{bbbbbbd} & \texttt{bbbbb\{b,d\}}\\
\textbf{Magenta} & {bbbbbbb} & {b\{b,d\}} & {bbbbb\{b,d\}} & {bbbbd} & {bbb\{\_,c,d\}}\\
%\textbf{Magenta} & \texttt{bbbbbbb} & \texttt{b\{b,d\}} & \texttt{bbbbb\{b,d\}} & \texttt{bbbbd} & \texttt{bbb\{\_,c,d\}}\\
\hline
\end{tabular}
\end{footnotesize}
%\caption{Messages most often used by the two agents when speaking about a given object. Brackets indicate variations often seen in the messages.}
%\label{tab:two_factors_messages}
\end{subfigure}

\vspace*{5mm}
\begin{subfigure}{\textwidth}
\centering
\captionsetup{width=.7\linewidth}
\begin{footnotesize}
\begin{tabular}{l|l|l|l|l|l}
\hline
\textbf{-} & \textbf{Box} & \textbf{Sphere} & \textbf{Cylinder} & \textbf{Capsule} & \textbf{Ellipsoid} \\
\hline
\textbf{Blue} & {- - - - -bb\{b,d\}} & {bb\{b,d\}} & {- - - -bb\{b,d\}} & {- - -bb\{c,d\}} & {- -bb\{\_,c,d\}}\\
%\textbf{Blue} & \texttt{-----bb\{b,d\}} & \texttt{bb\{b,d\}} & \texttt{----bb\{b,d\}} & \texttt{---bb\{c,d\}} & \texttt{--bb\{\_,c,d\}}\\
\textbf{Red} & {++++\{c,e\}} & {++\{c,e\}} & {+++\{c,e\}} & {+\{c,e\}} & {\{c,e\}}\\
%\textbf{Red} & \texttt{++++\{c,e\}} & \texttt{++\{c,e\}} & \texttt{+++\{c,e\}} & \texttt{+\{c,e\}} & \texttt{\{c,e\}}\\
\textbf{White} & {- - - - -b} & {\{b,d\}} & {- - - -\{b,d\}} & {- - -\{b,d\}} & {- -\{\_,c,d\}}\\
%\textbf{White} & \texttt{-----b} & \texttt{\{b,d\}} & \texttt{----\{b,d\}} & \texttt{---\{b,d\}} & \texttt{--\{\_,c,d\}}\\
\textbf{Gray} & {++++**a} & {++**a} & {+++**a} & {+**c} & {**\{b,bd\}}\\
%\textbf{Gray} & \texttt{++++**a} & \texttt{++**a} & \texttt{+++**a} & \texttt{+**c} & \texttt{**\{b,bd\}}\\
\textbf{Yellow} & {++++aa} & {++aa} & {+++aa} & {+aa} & {a\{a,e\}}\\
%\textbf{Yellow} & \texttt{++++aa} & \texttt{++aa} & \texttt{+++aa} & \texttt{+aa} & \texttt{a\{a,e\}}\\
\textbf{Green} & {++++\{a,ad\}} & {++\{a,ad\}} & {+++\{a,ad\}} & {+\{a,ad\}} & {a}\\
%\textbf{Green} & \texttt{++++\{a,ad\}} & \texttt{++\{a,ad\}} & \texttt{+++\{a,ad\}} & \texttt{+\{a,ad\}} & \texttt{a}\\
\textbf{Cyan} & {a$\times$20} & {bbb\{b,d\}} & {- - - -bbb\{b,d\}} & {- - -bbbd} & {- -bbb\{b,d\}}\\
%\textbf{Cyan} & \texttt{a$\times$20} & \texttt{bbb\{b,d\}} & \texttt{----bbb\{b,d\}} & \texttt{---bbbd} & \texttt{--bbb\{b,d\}}\\
\textbf{Magenta} & {- - - - -bb} & {b\{b,d\}} & {- - - -b\{b,d\}} & {- - -bd} & {- -b\{\_,c,d\}}\\
%\textbf{Magenta} & \texttt{-----bb} & \texttt{b\{b,d\}} & \texttt{----b\{b,d\}} & \texttt{---bd} & \texttt{--b\{\_,c,d\}}\\
\hline
\end{tabular}
\end{footnotesize}
%\caption{Potential analysis of the messages in terms of prefixes and suffixes.}
%\label{tab:two_factors_analysis}
\end{subfigure}
%\caption{Messages most often used by the two agents when speaking about a given object. Brackets indicate variations often seen in the messages.}
\caption{(Top) Messages most often used by the two agents when speaking about a given object. Brackets indicate the variation often seen at the last character. Underscores indicate blanks. (Bottom) Potential analysis of the messages. \textit{Blue, White, Cyan, Magenta} start messages with \textit{b}'s while \textit{Red, Gray, Yellow, Green} start with \textit{a}'s. The asterisk indicates a negative \textit{a}.}
\label{tab:two_factors_analysis}
\end{table}

==> table_f2_16760.tex <==
\begin{table}[h]
% \small
\centering
\caption{Messages most often used by the two agents when speaking about a given object in round $16,760$ (training accuracy:$98.0\%$, agent0 perplexity:$0.57$, agent1 perplexity:$0.49$, Jaccard similarity:$0.82$). Brackets indicate the variation often seen at the last character. Underscores indicate blanks.}
\begin{footnotesize}
\begin{tabular}{l|l|l|l|l|l}
\hline
\textbf{-} & \textbf{Box} & \textbf{Sphere} & \textbf{Cylinder} & \textbf{Capsule} & \textbf{Ellipsoid} \\
\hline
\textbf{Blue} & {bbbbbbb\{b,d\}} & {bb\{b,d\}} & {bbbbbb\{b,d\}} & {bbbbb\{c,d\}} & {bbbb\{\_,c,d\}}\\
%\textbf{Blue} & \texttt{bbbbbbb\{b,d\}} & \texttt{bb\{b,d\}} & \texttt{bbbbbb\{b,d\}} & \texttt{bbbbb\{c,d\}} & \texttt{bbbb\{\_,c,d\}}\\
\textbf{Red} & {aaaa\{c,e\}} & {aa\{c,e\}} & {aaa\{c,e\}} & {a\{c,e\}} & {c,e}\\
%\textbf{Red} & \texttt{aaaa\{c,e\}} & \texttt{aa\{c,e\}} & \texttt{aaa\{c,e\}} & \texttt{a\{c,e\}} & \texttt{c,e}\\
\textbf{White} & {bbbbbb} & {b,d} & {bbbb\{b,d\}} & {bbb\{b,d\}} & {bb\{\_,c,d\}}\\
%\textbf{White} & \texttt{bbbbbb} & \texttt{b,d} & \texttt{bbbb\{b,d\}} & \texttt{bbb\{b,d\}} & \texttt{bb\{\_,c,d\}}\\
\textbf{Gray} & {aaa} & {a} & {aa} & {c} & {b,bd}\\
%\textbf{Gray} & \texttt{aaa} & \texttt{a} & \texttt{aa} & \texttt{c} & \texttt{b,bd}\\
\textbf{Yellow} & {aaaaaa} & {aaaa} & {aaaaa} & {aaa} & {a\{a,e\}}\\
%\textbf{Yellow} & \texttt{aaaaaa} & \texttt{aaaa} & \texttt{aaaaa} & \texttt{aaa} & \texttt{a\{a,e\}}\\
\textbf{Green} & {aaaa\{a,ad\}} & {aa\{a,ad\}} & {aaa\{a,ad\}} & {a\{a,ad\}} & {a}\\
%\textbf{Green} & \texttt{aaaa\{a,ad\}} & \texttt{aa\{a,ad\}} & \texttt{aaa\{a,ad\}} & \texttt{a\{a,ad\}} & \texttt{a}\\
\textbf{Cyan} & {a$\times$20} & {bbb\{b,d\}} & {bbbbbbb\{b,d\}} & {bbbbbbd} & {bbbbb\{b,d\}}\\
%\textbf{Cyan} & \texttt{a$\times$20} & \texttt{bbb\{b,d\}} & \texttt{bbbbbbb\{b,d\}} & \texttt{bbbbbbd} & \texttt{bbbbb\{b,d\}}\\
\textbf{Magenta} & {bbbbbbb} & {b\{b,d\}} & {bbbbb\{b,d\}} & {bbbbd} & {bbb\{\_,c,d\}}\\
%\textbf{Magenta} & \texttt{bbbbbbb} & \texttt{b\{b,d\}} & \texttt{bbbbb\{b,d\}} & \texttt{bbbbd} & \texttt{bbb\{\_,c,d\}}\\
\hline
\end{tabular}
\end{footnotesize}
\label{tab:two_factors_16760}
\end{table}

==> table_f2_19190.tex <==
\begin{table}[t]
% \small
\centering
\begin{subfigure}{\textwidth}
\centering
\captionsetup{width=.7\linewidth}
\begin{footnotesize}
\begin{tabular}{l|l|l|l|l|l}
\hline
\textbf{-} & \textbf{Box} & \textbf{Sphere} & \textbf{Cylinder} & \textbf{Capsule} & \textbf{Ellipsoid} \\
\hline
\textbf{Blue} & bbbbbb & bb & bbbbb & bbb\{b,bc\} & bb\{b,bc\}\\
\textbf{Red} & aaa\{a,ac\} & a\{a,ac\} & aa\{a,ac\} & a & c\\
\textbf{White} & bbbbd & d & bbbd & bbd & bd\\
\textbf{Gray} & aaa & a & aa & c & b\\
\textbf{Yellow} & aaaaaaa & aaaa\{a,e\} & aaaaaa & aaa\{a,e\} & aae\\
\textbf{Green} & aaaaaa & aaae & aaaae & aae & ac\\
\textbf{Cyan} & bbbbbbb & bbb & bbbbbb & bbbbb & bbbb\\
\textbf{Magenta} & bbbbb\{c,d\} & b\{,c\} & bbbb\{c,d\} & bbb\{c,d\} & bb\{c,d\}\\
\hline
\end{tabular}
\end{footnotesize}
%\caption{Messages most often used by the two agents when speaking about a given object. Brackets indicate variations often seen in the messages.}
%\label{tab:two_factors_messages}
\end{subfigure}

\vspace*{5mm}
\begin{subfigure}{\textwidth}
\centering
\captionsetup{width=.7\linewidth}
\begin{footnotesize}
\begin{tabular}{l|l|l|l|l|l}
\hline
\textbf{-} & \textbf{Box} & \textbf{Sphere} & \textbf{Cylinder} & \textbf{Capsule} & \textbf{Ellipsoid} \\
\hline
\textbf{Blue} & \texttt{----}bb & bb & \texttt{---}bb & \texttt{--}b\{b,bc\} & \texttt{-}b\{b,bc\}\\
\textbf{Red} & \texttt{+++}\{a,ac\} & \texttt{+}\{a,ac\} & \texttt{++}\{a,ac\} & *a & **c\\
\textbf{White} & \texttt{----}d & d & \texttt{---}d & \texttt{--}d & \texttt{-}d\\
\textbf{Gray} & \texttt{+++} & \texttt{+} & \texttt{++} & *c & **b\\
\textbf{Yellow} & \texttt{+++}aaaa & \texttt{+}aaa\{a,e\} & \texttt{++}aaaa & *aaa\{a,e\} & **aae\\
\textbf{Green} & \texttt{+++}aaa & \texttt{+}aae & \texttt{++}aae & *aae & **ac\\
\textbf{Cyan} & \texttt{----}bbb & bbb & \texttt{---}bbb & \texttt{--}bbb & \texttt{-}bbb\\
\textbf{Magenta} & \texttt{----}b\{c,d\} & b\{,c\} & \texttt{---}b\{c,d\} & \texttt{--}b\{c,d\} & \texttt{-}b\{c,d\}\\
\hline
\end{tabular}
\end{footnotesize}
%\caption{Potential analysis of the messages in terms of prefixes and suffixes.}
%\label{tab:two_factors_analysis}
\end{subfigure}
%\caption{Messages most often used by the two agents when speaking about a given object. Brackets indicate variations often seen in the messages.}
\caption{(Top) Messages most often used by the two agents when speaking about a given object. Brackets indicate variations often seen in the messages. (Bottom) Potential analysis of the messages in terms of prefixes and suffixes. \textit{Blue, White Cyan} and \textit{Magenta} share the same prefixes, and the remaining colors also share the same prefixes. Asterisk indicates a negative prefix \textit{a}.}
\label{tab:two_factors_analysis}
\end{table}

==> table_f2_40.tex <==
\begin{table}[h]
% \small
\centering
\caption{Messages used by the two agents when speaking about any object in round 40 (training accuracy:$66.1\%$, agent0 perplexity:$0.0$, agent1 perplexity:$0.0$, Jaccard similarity:$0.0$).}
\begin{footnotesize}
\begin{tabular}{c|c|c}
\hline
\textbf{-} & \textbf{All objects described by Agent 0} & \textbf{All objects described by Agent 1}\\
\hline
\textbf{Message} & {dddddddddddddddddddd} & {bbbbbbbbbbbbbbbbbbbb}\\
\hline
\end{tabular}
\end{footnotesize}
\label{tab:two_factors_40}
\end{table}

==> table_f2_4400.tex <==
\begin{table}[h]
% \small
\centering
\begin{footnotesize}
\begin{tabular}{c|c|c}
\hline
\textbf{-} & \textbf{All objects described by Agent 0} & \textbf{All objects described by Agent 1}\\
\hline
\textbf{Message} & {aaaaaaaaaaaaaaaaaaaa} & {aaaaaaaaaaaaaaaaaaaa}\\
\hline
\end{tabular}
\end{footnotesize}
\caption{Messages used by the two agents when speaking about any object in round 4400 (training accuracy:$66.5\%$, agent0 perplexity:$0.0$, agent1 perplexity:$0.0$, Jaccard similarity:$1.0$). Both agents agreed to use \textit{aaaaaaaaaaaaaaaaaaaa} to describe all objects.}
\label{tab:two_factors_analysis_4400}
\end{table}

==> table_f2_6940.tex <==
\begin{table}[h]
% \small
\centering
\caption{Ten most frequent messages used by each agent to describe a \textit{red sphere} in round $6,940$ (training accuracy:$93.1\%$, agent0 perplexity:$10.94$, agent1 perplexity:$17.21$, Jaccard similarity:$0.0$).
%Both agents have not yet learned to single out the red sphere in the image, and are heavily affected by pixel-level differences between different images of a red sphere.
}
\begin{footnotesize}
\begin{tabular}{c|c|c}
\hline
\textbf{-} & \textbf{Red sphere described by agent 0} & \textbf{Red sphere described by agent 1}\\
\hline
\textbf{Messages} 
& \begin{tabular}{@{}c@{}}
aeceaeaeaaaeeeeeeeee\\
aacceeaaaaeeeeeeeeee\\
aaccceaaaaaaaaeeeeee\\
aeeeeaaaaeeeeeeeeeee\\
aeaceeaeaeeeeeeeeeee\\
aceacacaaaaaaeeeeeee\\
abeeeeaeeeeeeeeeeeee\\
aacceeaeeeeeeeeeeeee\\
aacceeaeaaeeeeeeeeee\\
aeeacacaaaeeccceeeee\\
%aeeacacaaaaaeeeeeeee\\
%aeceaeaaaeeeeeeeeeee\\
%aaeeeaaeaaaeaaaeeeee\\
%aaeecaacaaaaaaaaaaac\\
%aaeceeaaaaaeaeeeeeee\\
%aaeceacaaaaaaaaeaeee\\
%aacecaeaaeaaaeeeceee\\
%aacceacaacaaaaeeeeee\\
%aacccacaaaaaaaaeeecc\\
%aacbeeeaeaaeeeeeeeee\\
%aacbeeaeaaaeeeeeeeee\\
%aabceeaaeaaaeeeeeeee\\
%aabcceaeaaeccceeeeee\\
%aeeeacaaacceeeeeeeee\\
%aeeaeeaaaceeeeeeeeee\\
%aaeeccaaacaaaaaeeeee\\
%aaeecacaaaacaaaaeeee\\
%aaeecacaaaaaacccccee\\
%aaeeaccaaaaaaaaaaaac\\
%aaeceeaeaaaeeeeeeeee\\
%aaeceeaacceeeeeeeeee\\
%aaeceeaaaaaaaaaaaaaa\\
%aaceeacaaaaaaaaeeeee\\
%aaccceaeaaaaaeeeeeee\\
%aaccceaaeeeeeeeeeeee\\
%aabcceaaaaaaaeeeeeee\\
%aaabcdecaaaeaaaaaaee\\
%aeeeaeaeaeeeeeeeeeee\\
%aeceeaeaeeeeeeeeeeee\\
%aeceaeeaaeeeeeeeeeee\\
%acceeaaaeeeeeeeeeeee\\
%aaceeaeaaaaaaeeeeeee\\
%aacceeeaaeeeeeeeeeee\\
%aaccecaaaaaaaaaeeeec\\
%aacceacaaaaaaaaaeeee\\
%aaccceeaaaeeeeeeeeee\\
%aaccceaacaaeeeeeeeee\\
%aaccceaaacaaaeeeeeee\\
%aaccccaaaaaaaceeeeee\\
%aacbeeacaeecceeeeeec\\
\end{tabular} 
& \begin{tabular}{@{}c@{}}
aaedacacaaaaaaaaaaaa\\
aaccdaacaaaaaaaaaaaa\\
aaabcdadaaaaaaaaaaaa\\
aaeeacaeaaaaaaaaaaaa\\
aaccdadaaaaaaacaaaaa\\
aaedaceaaaaaaaaaaaaa\\
aaeaccaeaaaaaaaaaaaa\\
aaceacaacaaaaaaaaaaa\\
aacdacdaaaaaaaaaaaaa\\
aaccdadaaaaacaaaaaaa\\
%aaccdadaaaaaacaaaaaa\\
%aacdeaacaaaaacaaaaaa\\
%aacdeaacaaaaaaaaaaaa\\
%aacddaeaaaacaaaaaaaa\\
%aacddacaaaaaaaaaaaaa\\
%aacddaacaaaaaaaaaaaa\\
%aaccdadaacaacaaaaaac\\
%aeaceaacaaaacaaacaaa\\
%aeacdaacaaaaaaaaacaa\\
%aeaccacaacaacaaacaaa\\
%adeacacaaacaacaacaac\\
%aacddaeaaaaaaaaaaaaa\\
%aacdacaeaaaaaaaaaaaa\\
%aaccacdaaaaaaaaaaaaa\\
%aeeadacaacaaaaaacaaa\\
%aeacddaaacaaaaacaaaa\\
%aeacddaaaaaacaaaacaa\\
%aaeeadaeaaaaaaaaaaaa\\
%aaeeaceaaaaaaaaaaaaa\\
%aaeeacacaaaaaaaaaaaa\\
%aaedeaeaaaaaaaaaaaaa\\
%aaedeaacaaaaaaaaaaaa\\
%aaeaccaaeaaaaaaaaaaa\\
%aacdacacaaaaaaaaaaaa\\
%aaccdadaaaaaaaaaaaaa\\
%aaccdaadaaaaaaaaaaaa\\
%aaccdaacaaaaaacaaaaa\\
%aeeacacaaacacaacaaca\\
%aeacdaacaaaaacaaaaac\\
%aaceacacaaaaaaaaaaaa\\
%aacceaadaaaaaaaaaaac\\
%aaccdadaaaaaaaaaacaa\\
%aaccdaaaeaaaaaacaaaa\\
%aeeaddaacaacaacaaaca\\
%aeeadacaacaaacaaaaaa\\
%aeacdadaacaacaaaaaca\\
%aeacdacacaaaacaaacaa\\
%aaeeaddaaaaaaaaaaaaa\\
%aaeeadacaaaaaaaaaaaa\\
%aaeeacdaaaaaaaaaaaaa\\
\end{tabular}\\
\hline
\end{tabular}
\end{footnotesize}
\label{tab:two_factors_6940}
\end{table}

==> table_f2_analysis_16760.tex <==
\begin{table}[h]
% \small
\centering
\caption{(Top) Potential composition analysis of the messages from round 16,760 (bottom of Table~\ref{tab:compositionality_comparison}). {+} and {-} respectively indicate consecutive \textit{a}'s and \textit{b}'s. The asterisk indicates a single deletion of \textit{a}. (Bottom) Rules for each color and shape derived from the top table.}
\begin{subfigure}{\textwidth}
\centering
\captionsetup{width=.7\linewidth}
\begin{footnotesize}
\begin{tabular}{l|l|l|l|l|l}
\hline
\textbf{-} & \textbf{Box} & \textbf{Sphere} & \textbf{Cylinder} & \textbf{Capsule} & \textbf{Ellipsoid} \\
\hline
\textbf{Blue} & {- - - - -bb\{b,d\}} & {bb\{b,d\}} & {- - - -bb\{b,d\}} & {- - -bb\{c,d\}} & {- -bb\{\_,c,d\}}\\
%\textbf{Blue} & \texttt{-----bb\{b,d\}} & \texttt{bb\{b,d\}} & \texttt{----bb\{b,d\}} & \texttt{---bb\{c,d\}} & \texttt{--bb\{\_,c,d\}}\\
\textbf{Red} & {++++\{c,e\}} & {++\{c,e\}} & {+++\{c,e\}} & {+\{c,e\}} & {\{c,e\}}\\
%\textbf{Red} & \texttt{++++\{c,e\}} & \texttt{++\{c,e\}} & \texttt{+++\{c,e\}} & \texttt{+\{c,e\}} & \texttt{\{c,e\}}\\
\textbf{White} & {- - - - -b} & {\{b,d\}} & {- - - -\{b,d\}} & {- - -\{b,d\}} & {- -\{\_,c,d\}}\\
%\textbf{White} & \texttt{-----b} & \texttt{\{b,d\}} & \texttt{----\{b,d\}} & \texttt{---\{b,d\}} & \texttt{--\{\_,c,d\}}\\
\textbf{Gray} & {++++**a} & {++**a} & {+++**a} & {+**c} & {**\{b,bd\}}\\
%\textbf{Gray} & \texttt{++++**a} & \texttt{++**a} & \texttt{+++**a} & \texttt{+**c} & \texttt{**\{b,bd\}}\\
\textbf{Yellow} & {++++aa} & {++aa} & {+++aa} & {+aa} & {a\{a,e\}}\\
%\textbf{Yellow} & \texttt{++++aa} & \texttt{++aa} & \texttt{+++aa} & \texttt{+aa} & \texttt{a\{a,e\}}\\
\textbf{Green} & {++++\{a,ad\}} & {++\{a,ad\}} & {+++\{a,ad\}} & {+\{a,ad\}} & {a}\\
%\textbf{Green} & \texttt{++++\{a,ad\}} & \texttt{++\{a,ad\}} & \texttt{+++\{a,ad\}} & \texttt{+\{a,ad\}} & \texttt{a}\\
\textbf{Cyan} & {a$\times$20} & {bbb\{b,d\}} & {- - - -bbb\{b,d\}} & {- - -bbbd} & {- -bbb\{b,d\}}\\
%\textbf{Cyan} & \texttt{a$\times$20} & \texttt{bbb\{b,d\}} & \texttt{----bbb\{b,d\}} & \texttt{---bbbd} & \texttt{--bbb\{b,d\}}\\
\textbf{Magenta} & {- - - - -bb} & {b\{b,d\}} & {- - - -b\{b,d\}} & {- - -bd} & {- -b\{\_,c,d\}}\\
%\textbf{Magenta} & \texttt{-----bb} & \texttt{b\{b,d\}} & \texttt{----b\{b,d\}} & \texttt{---bd} & \texttt{--b\{\_,c,d\}}\\
\hline
\end{tabular}
\end{footnotesize}
%\caption{Potential analysis of the messages in terms of prefixes and suffixes.}
%\label{tab:two_factors_analysis}
\end{subfigure}

\vspace*{5mm}
\begin{subfigure}{\textwidth}
\centering
\captionsetup{width=.7\linewidth}
\begin{footnotesize}
\begin{tabular}{l|l}
\multicolumn{2}{l}{Define \textit{Blue, White, Cyan, Magenta} as color group 0, rest as color group 1.} \\
\hline
\textbf{-} & \textbf{Rule}\\
\hline
\textbf{Blue} & End with \textit{bbb} or \textit{bbd}\\
\textbf{Red} & End with \textit{c} or \textit{e}\\
\textbf{White} & End with \textit{b} or \textit{d}\\
\textbf{Gray} & End with \textit{**a}\\
\textbf{Yellow} & End with \textit{aa}\\
\textbf{Green} & End with \textit{a} or \textit{ad}\\
\textbf{Cyan} & End with \textit{bbbb} or \textit{bbbd}\\
\textbf{Magenta} & End with \textit{bb} or \textit{bd}\\
\hline
\textbf{Box} & Start with \textit{bbbbb} for color group 0, start with \textit{aaaa} for color group 1\\
\textbf{Sphere} & Start with \textit{aa} for color group 1\\
\textbf{Cylinder} & Start with \textit{bbbb} for color group 0, start with \textit{aaa} for color group 1\\
\textbf{Capsule} & Start with \textit{bbb} for color group 0, start with \textit{a} for color group 1\\
\textbf{Ellipsoid} & Start with \textit{bb} for color group 0\\
\hline
\end{tabular}
\end{footnotesize}
%\caption{Potential analysis of the messages in terms of prefixes and suffixes.}
%\label{tab:two_factors_analysis}
\end{subfigure}
\label{tab:two_factors_analysis_16760}
\end{table}

==> table_f2_diagonal.tex <==
\begin{table}[h]
% \small
\centering
\begin{subfigure}{\textwidth}
\centering
\captionsetup{width=.7\linewidth}
\begin{footnotesize}
\begin{tabular}{l|l|l|l|l|l}
\hline
\textbf{-} & \textbf{Box} & \textbf{Sphere} & \textbf{Cylinder} & \textbf{Capsule} & \textbf{Ellipsoid} \\
\hline
\textbf{Blue} & \cellcolor{light_gray}eeeeeee\{e,ee\} & eeeeee & eeeeee\{e,ed\} & eeee\{e,ed\} & eee\{e,a\}\\
%\textbf{Blue} & \cellcolor{light_gray}\texttt{eeeeeee\{e,ee\}} & \texttt{eeeeee} & \texttt{eeeeee\{e,ed\}} & \texttt{eeee\{e,ed\}} & \texttt{eee\{e,a\}}\\
\textbf{Red} & ee\{e,a\} & \cellcolor{light_gray}e,ea & e\{e,a\} & {b,ba} & {a,c}\\
%\textbf{Red} & \texttt{ee\{e,a\}} & \cellcolor{light_gray}\texttt{e,ea} & \texttt{e\{e,a\}} & \texttt{b,ba} & \texttt{a,c}\\
\textbf{White} & {bbbbb} & {bb} & \cellcolor{light_gray}{bbb\{b,d\}} & {bb\{b,d\}} & {bbb\{d,c\}}\\
%\textbf{White} & \texttt{bbbbb} & \texttt{bb} & \cellcolor{light_gray}\texttt{bbb\{b,d\}} & \texttt{bb\{b,d\}} & \texttt{bbb\{d,c\}}\\
\textbf{Gray} & {eeee} & {e,ea} & {ee\{e,a\}} & \cellcolor{light_gray}{e,a} & {b,d}\\
%\textbf{Gray} & \texttt{eeee} & \texttt{e,ea} & \texttt{ee\{e,a\}} & \cellcolor{light_gray}\texttt{e,a} & \texttt{b,d}\\
\textbf{Yellow} & {bb\{c,d\}} & {e\{e,ec\}} & {b\{c,d\}} & {a,c} & \cellcolor{light_gray}{a,e}\\
%\textbf{Yellow} & \texttt{bb\{c,d\}} & \texttt{e\{e,ec\}} & \texttt{b\{c,d\}} & \texttt{a,c} & \cellcolor{light_gray}\texttt{a,e}\\
\textbf{Green} & {eeeeee\{e,a\}} & {eeee\{e,a\}} & {eeeee\{e,a\}} & {eee\{e,a\}} & {ee\{e,a\}}\\
%\textbf{Green} & \texttt{eeeeee\{e,a\}} & \texttt{eeee\{e,a\}} & \texttt{eeeee\{e,a\}} & \texttt{eee\{e,a\}} & \texttt{ee\{e,a\}}\\
\textbf{Cyan} & {eeeeeeeeea,a$\times$20}  & {eeeeee\{e,a\}} & {eeeeeee\{e,ea\}} & {eeeee\{e,a\}} & {eeeea}\\
%\textbf{Cyan} & \texttt{eeeeeeeeea,a$\times$20}  & \texttt{eeeeee\{e,a\}} & \texttt{eeeeeee\{e,ea\}} & \texttt{eeeee\{e,a\}} & \texttt{eeee\{e,a,c\}}\\
\textbf{Magenta} & {bbb\{b,d\}} & {c,d} & {bb\{b,d\}} & {bb} & {b\{c,a\}}\\
%\textbf{Magenta} & \texttt{bbb\{b,d\}} & \texttt{c,d} & \texttt{bb\{b,d\}} & \texttt{bb} & \texttt{b\{c,a\}}\\
\hline
\end{tabular}
\end{footnotesize}
%\caption{Messages most often used by the two agents when speaking about a given object. Brackets indicate variations often seen in the messages.}
%\label{tab:two_factors_messages}
\end{subfigure}

\vspace*{5mm}
\begin{subfigure}{\textwidth}
\centering
\captionsetup{width=.7\linewidth}
\begin{footnotesize}
\begin{tabular}{l|l|l|l|l|l}
\hline
\textbf{-} & \textbf{Box} & \textbf{Sphere} & \textbf{Cylinder} & \textbf{Capsule} & \textbf{Ellipsoid} \\
\hline
\textbf{Blue} & \cellcolor{light_gray}{++++++e\{e,ee\}} & {++++ee} & {+++++e\{e,ed\}} & {+++e\{e,ed\}} & {++e\{e,a\}}\\
%\textbf{Blue} & \cellcolor{light_gray}\texttt{++++++e\{e,ee\}} & \texttt{++++ee} & \texttt{+++++e\{e,ed\}} & \texttt{+++e\{e,ed\}} & \texttt{++e\{e,a\}}\\
\textbf{Red} & {++++++****\{e,a\}} & \cellcolor{light_gray}{++++****\{e,ea\}} & {+++++****\{e,a\}} & {+++****\{b,ba\}} & {++****\{a,c\}} \\
%\textbf{Red} & \texttt{++++++****\{e,a\}} & \cellcolor{light_gray}\texttt{++++****\{e,ea\}} & \texttt{+++++****\{e,a\}} & \texttt{+++****\{b,ba\}} & \texttt{++****\{a,c\}} \\
\textbf{White} & {- - - -b} & {- b} & \cellcolor{light_gray}{- - -\{b,d\}} & {- -\{b,d\}} & {- - -\{d,c\}}\\
%\textbf{White} & \texttt{----\{b,d\}} & \texttt{-b} & \cellcolor{light_gray}\texttt{---\{b,d\}} & \texttt{--\{b,d\}} & \texttt{---\{c,d\}}\\
\textbf{Gray} & {++++++***e} & {++++***\{\_,a\}} & {+++++***\{e,a\}} & \cellcolor{light_gray}{+++***\{e,a\}} & {++***\{b,d\}} \\
%\textbf{Gray} & \texttt{++++++***e} & \texttt{++++***\{\_,a\}} & \texttt{+++++***\{e,a\}} & \cellcolor{light_gray}\texttt{+++***\{e,a\}} & \texttt{++***\{b,d\}} \\
\textbf{Yellow} & {- - - -\&\&\{c,d\}} & {-\&\&e\{e,ec\}} & {- - -\&\&\{c,d\}} & {- -\&\&\{a,c\}} & \cellcolor{light_gray}{- - -\&\&\{a,e\}}\\
%\textbf{Yellow} & \texttt{----\&\&\{c,d\}} & \texttt{-\&\&ee} & \texttt{---\&\&\{c,d\}} & \texttt{--\&\&\{a,c\}} & \cellcolor{light_gray}\texttt{---\&\&\{a,e\}}\\
\textbf{Green} & {++++++\{e,a\}} & {++++\{e,a\}} & {+++++\{e,a\}} & {+++\{e,a\}} & {++\{e,a\}}\\
%\textbf{Green} & \texttt{++++++\{e,a\}} & \texttt{++++\{e,a\}} & \texttt{+++++\{e,a\}} & \texttt{+++\{e,a\}} & \texttt{++\{e,a\}}\\
\textbf{Cyan} & {++++++eeea} & {++++ee\{e,a\}} & {+++++ee\{e,ea\}} & {+++ee\{e,a\}} & {++eea}\\
%\textbf{Cyan} & \texttt{++++++eeea} & \texttt{++++ee\{e,a\}} & \texttt{+++++ee\{e,ea\}} & \texttt{+++ee\{e,a\}} & \texttt{++ee\{e,a,c\}}\\
\textbf{Magenta} & {- - - -\&\{b,d\}} & {-\&\{c,d\}} & {- - -\&\{b,d\}} & {- -\&b} & {- - -\&\&\{c,a\}}\\
%\textbf{Magenta} & \texttt{----\&\{b,d\}} & \texttt{-\&\{c,d\}} & \texttt{---\&\{b,d\}} & \texttt{--\&b} & \texttt{---\&\{c,a\}}\\
\hline
\end{tabular}
\end{footnotesize}
%\caption{Potential analysis of the messages in terms of prefixes and suffixes.}
%\label{tab:two_factors_analysis}
\end{subfigure}
%\caption{Messages most often used by the two agents when speaking about a given object. Brackets indicate variations often seen in the messages.}
\caption{(Top) Messages most often used by the two agents when speaking about a given object. Shaded cells indicate the objects not seen during the training. Brackets indicate the variation often seen at the last character. 
(Bottom) Potential analysis of the messages. \textit{Blue, Red, Gray, Green, Cyan} start messages with \textit{e}'s while \textit{White, Yellow, Magenta} start with \textit{b}'s. The asterisk and the ampersand respectively indicate negative \textit{e} and negative \textit{b}.}
\label{tab:two_factors_diagonal_analysis}
\end{table}

==> todo.tex <==
\begin{itemize}
\item Build a suffix(prefix?) tree so that we can see the structure of the messages. Is there an automatic way?
\item Longest common subsequence. This could be another way to find structure in the messages.
\item 2-D embedding of the messages (MDS?). For all messages pairs, create a distance matrix. Do a PCA on it, take the two principal components, draw it on the 2D plane, annotate with object types. See if similar objects stick together.
\item Success/failure analysis, especially for zero-shots. If agents succeed, when and why? If they fail, when and why?
\end{itemize}
